On the choosability with separation of planar graphs and its correspondence colouring analogue

A list assignment $L$ for a graph $G$ is an $(\ell,k)$-list assignment if $|L(v)|\geq \ell$ for each $v \in V(G)$ and $|L(u) \cap L(v)| \leq k$ for each $uv \in E(G)$. We say $G$ is $(\ell,k)$-choosable if it admits an $L$-colouring for every $(\ell, k)$-list assignment $L$. We prove that if $G$ is a planar graph with $(4,2)$-list assignment $L$ and for every triangle $T \subseteq G$ we have that $|\bigcap_{v \in V(T)} L(v)| \neq 2$, then $G$ is $L$-colourable. In fact, we prove a slightly stronger result: if $G$ contains a clique $H$ such that $V(H) \cap V(T) \neq \emptyset$ for every triangle $T \subseteq G$ with $|\bigcap_{v \in V(T)} L(v)| = 2$, then $G$ is $L$-colourable. Additionally, we give a counterexample to the correspondence colouring analogue of $(4,2)$-choosability for planar graphs.

==> fig1.tex <==
\begin{figure}[ht]
\begin{center}
\begin{tikzpicture}[scale=0.72, invisnode/.style={circle, draw=white, fill=white,  minimum size=1mm}, blcknd/.style={inner sep=1pt, minimum size=8pt, circle,draw,fill}]
\node[blcknd, label={above:\{a\}}] at (0,2) (v1) {\color{white}$v_1$};
\node[blcknd, label={below:\{b\}}] at (0,-2) (v2) {\color{white}$v_2$};
\node[blcknd, label={left:\{a,b,1\}}] at (-4,0) (v3) {\color{white}$v_3$};
\node[blcknd, label={right:\{a,b,1\}}] at (4,0) (v4) {\color{white}$v_4$};

\node[] at (0,.4) {1};
\node[] at (2, 1.4) {a};
\node[] at (-2, 1.4) {a};
\node[] at (2,-1.5) {b};
\node[] at (-2,-1.5) {b};

\draw[black] (v1)--(v3);
\draw[black] (v2)--(v3);
\draw[black] (v3)--(v4);
\draw[black] (v1)--(v4);
\draw[black] (v2)--(v4);
\end{tikzpicture}
\end{center}
\caption{The gadget used in the proof of Theorem \ref{ctx31}. The list of each vertex is indicated in braces beside the vertex. A colour $c$ is indicated over an edge $e = uv$ iff $c \in M_{uv}$.}
    \label{fig:31}
\end{figure}


